Visual Programming: Compositional visual reasoning without training

We present VISPROG, a neuro-symbolic approach to solving complex and compositional visual tasks given natural language instructions. VISPROG avoids the need for any task-specific training. Instead, it uses the in-context learning ability of large language models to generate python-like modular programs, which are then executed to get both the solution and a comprehensive and interpretable rationale. Each line of the generated program may invoke one of several off-the-shelf computer vision models, image processing routines, or python functions to produce intermediate outputs that may be consumed by subsequent parts of the program. We demonstrate the flexibility of VISPROG on 4 diverse tasks - compositional visual question answering, zero-shot reasoning on image pairs, factual knowledge object tagging, and language-guided image editing. We believe neuro-symbolic approaches like VISPROG are an exciting avenue to easily and effectively expand the scope of AI systems to serve the long tail of complex tasks that people may wish to perform.

==> figs/program.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{imgs/program_shaded.png}

   \caption{\textbf{Program specification for generation.} Green shows the input used to initialize the program state, blue denotes the output variables, and magenta shows input values that are generated as part of the program. Note that output variables of past steps may be input to the current step. The generated program syntax is motivated by readability and ease of parsing but it is easy to use other conventions in \model\ by modifying the \textit{parse} method in the modules (Code.~\ref{lst:module}).}
   \label{fig:program}
\end{figure}

==> intro_v1.tex <==
The pursuit of building intelligent systems is a never-ending one. As soon as we build a system that can solve a set of complex tasks, it is usually trivial to increase the task complexity beyond the training distribution by composing these tasks in novel ways. In this work, we propose a vision system, \model, that deconstructs complex tasks into a sequence of simpler steps that the system is already trained to handle and produce a solution by reasoning about the outputs of these intermediate steps. 

Inference in \model\ involves writing and executing \textit{visual programs} that invoke predefined python functions (more generally, subroutines in any programming language) at intermediate steps to perform a complex visual task. For instance, as shown in \todo{ref teaser fig}, given a natural language instruction such as ``Tag the 7 main characters on the TV show Big Bang Theory.", \model\ first generates a visual program, a sequence of \textit{steps} such as - detect faces, retrieve list of main characters on Big Bang Theory from a knowledge base, classify faces using the list of characters, and tag the image with recognized character faces and their names. Each step involves specifying a function, function inputs or arguments, and the name of the variable to store the output. The output variable from the current step may be used as an input for subsequent steps. \model\ uses \gpt\ to generate the program given the instruction using a handful of in-context examples as a prompt. State-of-the-art modules (neural or otherwise) may be used to implement the \textit{step} functions, in this case - a face detector, \gpt\ as a knowledge retrieval system, and \clip\ as an open-vocabulary image classifier. 

\model\ is not the first model to generate and execute programs for vision applications. For the visual question answering (VQA) task, Neural Module Networks (NMN) and End-to-End Neural Module Networks (N2NMN)\todo{cite NMN, N2NMN, and justin johnsons inferring and executing programs} compose a question-specific, end-to-end trainable networks from specialized, differentiable neural modules. These approaches either use brittle, off-the-shelf semantic parsers to deterministically compute the layout, or learn a generator to predict the layout of modules through weak answer supervision via \reinf. In contrast, \model\ uses a powerful language model (\gpt) and a small number of in-context examples to create complex programs \textit{without} requiring any finetuning. Unlike previous approaches that compose a network that needs to be trained on the task, \model\ allows creating programs that invoke trained state-of-the-art models creating a performant, modular, and interpretable neuro-symbolic system. 

\model\ is interpretable at two levels. First, \model\ produces highly interpretable programs which a user can verify for algorithmic correctness. Second, a user can easily inspect the output of intermediate steps to diagnose errors in intermediate modules and if required, intervene in the reasoning process. Altogether, an executed program with intermediate step results serve as a \textit{visual rationale} for the prediction.  

To demonstrate its flexibility, we use \model\ for 4 different tasks sharing many modules across tasks. These tasks are - (i) compositional visual question answering; (ii) zero-shot natural language visual reasoning on image pairs; (iii) factual knowledge object tagging from natural language instructions; and (iv) language guided image editing. We did not finetune either the language model or the modules for any of these tasks. Adapting \model\ to any task is as simple as defining task-specific python functions and providing a few in-context examples consisting of natural language instructions and the corresponding programs that demonstrate use of these functions.

==> table/modules.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\resizebox{0.9\columnwidth}{!}{\begin{tabular}{lllc}
\toprule
\textbf{Function}                                                                 & \textbf{Module} & \textbf{Models / Subroutines}                                                           & \textbf{Neural}       \\
\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}Image\\ Understanding\end{tabular}}    & LOC             & OWL-ViT                                                                                 & \cmark \\
                                                                                  & FACEDET         & DSFD (pypi)                                                                                    & \cmark \\
                                                                                  & SEG             & MaskFormer                                                                              & \cmark \\
                                                                                  & SELECT          & CLIP-ViT                                                                                & \cmark \\
                                                                                  & VQA             & ViLT                                                                                    & \cmark \\ \hline
\multirow{9}{*}{\begin{tabular}[c]{@{}l@{}}Image\\ Manipulation\end{tabular}}     & CROP            & PIL.Image.crop()                                                                        & \xmark \\
                                                                                  & CROP-LEFTOF    & PIL.Image.crop()                                                                        & \xmark \\
                                                                                  & CROP-RIGHTOF   & PIL.Image.crop()                                                                        & \xmark \\
                                                                                  & CROP-ABOVE     & PIL.Image.crop()                                                                        & \xmark \\
                                                                                  & CROP-BELOW     & PIL.Image.crop()                                                                        & \xmark \\
                                                                                  & COLORPOP        & \begin{tabular}[c]{@{}l@{}}PIL.Image.convert()\\ cv2.grabCut()\end{tabular}             & \xmark \\
                                                                                  & BGBLUR          & \begin{tabular}[c]{@{}l@{}}PIL.ImageFilter.GaussianBlur()\\ cv2.graphCut()\end{tabular} & \xmark \\
                                                                                  & REPLACE         & StableDiffusion                                                                         & \cmark \\
                                                                                  & EMOJI           & AugLy (pypi)                                                                            & \xmark \\ \hline
\begin{tabular}[c]{@{}l@{}}Knowledge\\ Retrieval\end{tabular}                     & LIST            & GPT3                                                                                    & \cmark \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Arithmetic \\ \& Logical\end{tabular}} & EVAL            & eval()                                                                                  & \xmark \\
                                                                                  & COUNT           & len()                                                                                   & \xmark \\
\bottomrule
\end{tabular}}
\end{table}
